Make life simple: unleash the full power of the parallel tempering algorithm

We introduce a new update scheme to systematically improve the efficiency of parallel tempering simulations. We show that by adapting the number of sweeps between replica exchanges to the canonical autocorrelation time, the average round-trip time of a replica in temperature space can be significantly decreased. The temperatures are not dynamically adjusted as in previous attempts but chosen to yield a 50% exchange rate of adjacent replicas. We illustrate the new algorithm with results for the Ising model in two and the Edwards-Anderson Ising spin glass in three dimensions

==> Makefile <==
.PHONY:all clean
	
LATEX=latex
DVIPDF=dvipdf

SOURCES=pt_draft.tex
EPS=eta_and_tunnel.eps tau_80.eps tunnelingtimes_80.eps flow.eps temp_walk_3.eps 
TOOLS=Makefile psfig.sty

all: $(SOURCES:.tex=.pdf)

clean:
	rm -f *.aux *.log

.tex.dvi:
	$(LATEX) --interaction nonstopmode $< | clean_tex
	$(LATEX) --interaction nonstopmode $< | clean_tex

%.pdf: %.dvi
	$(DVIPDF) $<

tar:
	@D=`date '+%d_%m_%y'`; \
	tar -czf "pt_opti_$${D}.tar.gz" $(SOURCES) $(EPS) $(TOOLS); 


